Dolphin: An Actor-Oriented Database for Reactive Moving Object Data Management

Novel reactive moving object applications require solutions to support object reactive behaviors as a way to query and update dynamic data. While moving object scenarios have long been researched in the context of spatio-temporal data management, reactive behavior is usually left to complex end-user implementations. However, it is not just a matter of hardwiring reactive constraints: the required solutions need to satisfy tight low-latency computation requirements and be scalable. This paper explores a novel approach to enrich a distributed actor-based framework with reactive functionality and complex spatial data management along with concurrency semantics. Our approach relies on a proposal of the moving actor abstraction, which is a conceptual enhancement of the actor model with reactive sensing, movement, and spatial querying capabilities. This enhancement helps developers of reactive moving object applications avoid the significant burden of implementing application-level schemes to balance performance and consistency. Based on moving actors, we define a reactive moving object data management platform, named Moving Actor-Oriented Databases (M-AODBs), and build Dolphin -- an implementation of M-AODBs. Dolphin embodies a non-intrusive actor-based design layered on top of the Microsoft Orleans distributed virtual actor framework. In a set of experimental evaluations with realistic reactive moving object scenarios, Dolphin exhibits scalability on multi-machines and provides near-real-time reaction latency.

==> 2_Example.tex <==
\vspace{-0.2cm}
\section{Reactive Moving Object Applications}
\label{sec:examples}

\subsection{Examples of Reactive Moving Object Applications}
The number of reactive moving object applications continues to increase, e.g.,  fleet management~\citep{sorensen2010conceptual,burgard2000collaborative}, multi-robot collaborative systems~\citep{agriculturalfuture,albani2017monitoring,smartfarmingIoT},  location-aware trans-reality games~\citep{gutierrez2012faars,lindley2005narrative}, or potential criminal trajectory tracking systems~\citep{abd2012gis, elrefaei2017real, tundis2020detecting},
%Those systems supervise the use and maintenance of machines or robots to coordinate and disseminate tasks and collect information to solve heterogeneous scheduling and routing problems. In social network applications, people can receive notifications if there are interests spots or friends in their subscribe range~\citep{stephen202023,capponi2019survey}.
%Location-aware trans-reality games~\citep{gutierrez2012faars,lindley2005narrative} %players moves in the real or virtual spaces where navigating through the environment is one of the most common activities. 
%MMO games provides reactive mechanisms that can be triggered by interaction between reality and players' movements. %Despite of virtual or real space interaction, all actions of players will be ingested into server side, It is non-trival task to allow for unmatched information collection as different granularity levels and completeness of collected information. 
%In potential criminal trajectory tracking systems~\citep{abd2012gis, elrefaei2017real, tundis2020detecting}, alerts are raised and notification are send to law enforcement agents when supervised targets approach potential victims or specific areas that they do not allow to.

\begin{wrapfigure}{l}
 \centering 
  \vspace{-0.5cm}
  \includegraphics[scale=0.13]{images/c-itsexample.pdf}
  \hspace{-.3in}
  \vspace{0.7cm}
  \caption{C-ITS Example}
  \label{fig:citsexample}
  \vspace{-0.4cm}
  %https://docs.google.com/drawings/d/1TKja-0tGIo8DWrVqgpvLC3lOeZ8_hJvidhVwkloxz4M/edit?usp=sharing
\end{wrapfigure}
\hspace{-0.3cm}
Our case study concerns a particular kind of application --  Cooperative Intelligent Transportation Systems (C-ITS) \citep{mitsakis2020c, bussche2020hedging, nguyen2020towards}, in which vehicles communicate and cooperate towards improving overall transportation effectiveness, driving behaviours, security and safety \citep{ni2016traffic}. 
While regular ITS \citep{papp2008world, DBLP:journals/itsm/LiN13, hu2020cooperative, tak2020sectional} concentrate on local information sharing, optimization and coordination (\textit{e.g.}, involving drivers, traffic controllers, or transportation system operators) to make better decisions, in C-ITS, global information ingestion is required and vehicles themselves are active participants in transportation actions and decisions. 
Figure \ref{fig:citsexample} presents an example of C-ITS. 
Reactive vehicles (shown as red vehicle icons) start reactive sensing within  a specific spatial region (shown as a semi-transparent red range). %-- here called its \emph{reactive sensing area}. 
A reactive vehicle is aware of other vehicles if those vehicles' movements satisfy its predefined spatial predicates  (e.g., cross, cover, or overlap) against its spatial sensing area. 
Predicates may vary from vehicle to vehicle. In a simplified way, in standard ITS vehicle behavior is managed by the application, whereas in C-ITS vehicles are active participants in deciding their movements.
Thus, a reactive vehicle can take reactive actions,  such as communication with approaching vehicles to send warnings to help them avoid hazards~\citep{Uhlemann18:ConnectedVehicles}. 
In the future,  cooperation will be a critical ingredient for self-driving or assisted-driving.
%C-ITS driving provides benefits to both drivers and vehicle's automation.

%The behavioural planner or decision-maker provides ad-hoc decisions by using interaction information with other moving objects. 

\vspace{-0.3cm}
\subsection{Reactive Moving Object Data Management Requirements}
\label{sec:reqs}
Those novel reactive moving object applications require specific data management system solutions. 
We summarize below the 4 main requirements for a desired reactive moving object data management system.


%\begin{enumerate}[label=\subscript{Req}{{\arabic*}}]
    \noindent\textbf{Req 0. Support the Non-reactive Requirements of Spatial Data Management}: reactive moving object data management systems require support to traditional spatial operations like spatial queries and updates, and maintenance of spatial static integrity constraints.

    \noindent\textbf{Req 1. Support and Represent Concurrent Heterogeneous Moving Objects}: a reactive moving object data management system should treat each moving object independently and support their concurrent behaviour. %It is, however, convenient to model objects by type and collaboration behavior.
    It should allow modeling objects by type and collaboration behavior.
    \label{req1}

    \noindent\textbf{Req 2. Support Spatial Reactive Behavior}: a reactive moving object data management system should support reactive objects. These objects must be able to sense their surroundings or other areas of space to perform reactive actions. This requires to efficiently process reactive behaviour  among objects that are triggered by their surrounding objects and environment. 
    \label{req2}
    
    \noindent\textbf{Req 3. Provide Scalability and Elasticity}: a reactive moving object data management system should scale to arbitrary numbers of objects while supporting the processing of complex space-dependent application logics. Additionally, a reactive moving object is a digital twin of a real-world entity. Its lifecycle should be the same that of the corresponding real world entity as it enters and/or leaves the system. Since load vary dynamically depending on the relative positions of moving objects, the system should manage underlying resources elastically. 
    \label{req3}

    %\noindent\textbf{Req 4. Be Resilient to Spatial Skew}: a reactive moving object data management system should handle skew in the distribution of objects in space to mitigate degradation in performance and keeps scalability when objects are clustered. 
    %\label{req4}
%\end{enumerate}

